Black-Box Targeted Reward Poisoning Attack Against Online Deep Reinforcement Learning

We propose the first black-box targeted attack against online deep reinforcement learning through reward poisoning during training time. Our attack is applicable to general environments with unknown dynamics learned by unknown algorithms and requires limited attack budgets and computational resources. We leverage a general framework and find conditions to ensure efficient attack under a general assumption of the learning algorithms. We show that our attack is optimal in our framework under the conditions. We experimentally verify that with limited budgets, our attack efficiently leads the learning agent to various target policies under a diverse set of popular DRL environments and state-of-the-art learners.

==> figures/HalfCheetah_baseline.tex <==
\begin{figure}[!ht]
\centering
\includegraphics[width=0.7\linewidth]{figures/HalfCheetah_baseline.png}

\caption{Training log for adaptive target attack and neighborhood target attack in HalfCheetah with a hard limit on budget $\frac{C}{T}=7.5$}
\label{fig:HCb}
\end{figure}

==> figures/HalfCheetah_log.tex <==
\begin{figure}[!ht]
\centering
\includegraphics[width=0.7\linewidth]{figures/HalfCheetah_log.png}

\caption{Training log for HalfCheetah environment under no attack and adaptive target attack with $\Delta=50$.}
\label{fig:HCl}
\end{figure}

==> figures/MountainCar_baseline.tex <==
\begin{figure}[!ht]
\centering
\includegraphics[width=0.7\linewidth]{figures/MountainCar_baseline.png}

\caption{Training log for adaptive target attack and greedy target attack in MountainCar with a hard limit on budget $\frac{C}{T}=0.3$}
\label{fig:MCb}
\end{figure}

==> figures/MountainCar_log.tex <==

\begin{figure}[!ht]
\centering
\includegraphics[width=0.7\linewidth]{figures/MountainCar_log.png}

\caption{Training log for MountainCar environment under no attack and adaptive target attack with $\Delta=5$.}
\label{fig:MCl}
\end{figure}
